CoDiNet: Path Distribution Modeling with Consistency and Diversity for Dynamic Routing

Dynamic routing networks, aimed at finding the best routing paths in the networks, have achieved significant improvements to neural networks in terms of accuracy and efficiency. In this paper, we see dynamic routing networks in a fresh light, formulating a routing method as a mapping from a sample space to a routing space. From the perspective of space mapping, prevalent methods of dynamic routing didn't consider how inference paths would be distributed in the routing space. Thus, we propose a novel method, termed CoDiNet, to model the relationship between a sample space and a routing space by regularizing the distribution of routing paths with the properties of consistency and diversity. Specifically, samples with similar semantics should be mapped into the same area in routing space, while those with dissimilar semantics should be mapped into different areas. Moreover, we design a customizable dynamic routing module, which can strike a balance between accuracy and efficiency. When deployed upon ResNet models, our method achieves higher performance and effectively reduces average computational cost on four widely used datasets.

==> sections/reference.tex <==
\begin{thebibliography}{1}
	
	% \bibitem{li2019improved}
	% Hao, Li and Hong, Zhang and Xiaojuan, Qi and Ruigang, Yang and Gao, Huang,
	% Improved Techniques for Training Adaptive Deep Networks.
	% Proceedings of the International Conference on Computer Vision, {ICCV}
	% (2019)
	
	% \bibitem{veit2018convolutional}
	% Andreas, Veit and Serge, J. Belongie,
	% Convolutional networks with adaptive inference graphs.
	% Proceedings of the European Conference on Computer Vision, {ECCV}
	% (2018)
	
	% \bibitem{wang2018skipnet}
	% Xin, Wang and Fisher, Yu and Zi-Yi, Dou and Trevor, Darrell and Joseph, E. Gonzalez,
	% Skipnet: Learning dynamic routing in convolutional networks,
	% Proceedings of the European Conference on Computer Vision, {ECCV} 
	% (2018)
	
	% \bibitem{wu2018blockdrop}
	% Zuxuan, Wu and Tushar, Nagarajan and Abhishek, Kumar and Steven, Rennie and Larry, S. Davis and Kristen, Grauman and Feris, Rogerio,
	% Blockdrop: Dynamic inference paths in residual networks,
	% Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, {CVPR}
	% (2018)
	
	% \bibitem{cai2019once}
	% Han, Cai and	Chuang, Gan and Tianzhe, Wang and Zhekai, Zhang and Song, Han,
	% Once for all: Train one network and specialize it for efficient deployment,
	% Proceedings of the International Conference on Learning Representations, {ICLR}
	% (2020)
	
	% \bibitem{EnsemblesShallow}
	% Veit, Andreas and Wilber, Michael and Belongie, Serge,
	% Residual Networks Behave like Ensembles of Relatively Shallow Networks,
	% Proceedings of the International Conference on Neural Information Processing Systems, {NIPS}
	% (2016)
	
	% \bibitem{ochsner2004better}
	% Ochsner, Kevin N and Ray, Rebecca D and Cooper, Jeffrey C and Robertson, Elaine R and Chopra, Sita and Gabrieli, John DE and Gross, James J
	% For better or for worse: neural systems supporting the cognitive down-and up-regulation of negative emotion,
	% Neuroimage,
	% (2004)

	% \bibitem{Huang2017MultiScaleDN}
	% Gao, Huang and Danlu, Chen and Tianhong, Li and Felix, Wu and Laurens, van der Maaten and Kilian, Q. Weinberger,
	% Multi-Scale Dense Networks for Resource Efficient Image Classification,	
	% Proceedings of the International Conference on Learning Representations, {ICLR}
	% (2017)
	
	% \bibitem{huang2017densely}
	% Huang, Gao and Liu, Zhuang and van, der Maaten Laurens and Weinberger, Kilian Q,
	% Densely Connected Convolutional Networks,
	% Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, {CVPR}
	% (2017)
	
	\bibitem{figurnov2017spatially}
	Figurnov, Michael and Collins, Maxwell D and Zhu, Yukun and Zhang, Li and Huang, Jonathan and Vetrov, Dmitry and Salakhutdinov, Ruslan,
	Spatially adaptive computation time for residual networks,
	Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, {CVPR}
	(2017)
	
	\bibitem{graves2016adaptive}
	Graves, Alex,
	Adaptive computation time for recurrent neural networks,
	arXiv preprint arXiv:1603.08983
	(2016)
	
	\bibitem{yu2018slimmable}
	Yu, Jiahui and Yang, Linjie and Xu, Ning and Yang, Jianchao and Huang, Thomas,
	Slimmable neural networks,
	Proceedings of the International Conference on Learning Representations, {ICLR}
	(2018)
	
	\bibitem{reyzin2011boosting}
	Reyzin, Lev,
	Boosting on a budget: Sampling for feature-efficient prediction,
	Proceedings of the International Conference on Machine Learning, {ICML}
	(2011)
	
	\bibitem{odena2017changing}
	Odena, Augustus and Lawson, Dieterich and Olah, Christopher,
	Changing model behavior at test-time using reinforcement learning,
	Proceedings of the International Conference on Learning Representations Workshops, {ICLR Workshop}
	(2017)
	
	\bibitem{mcintosh2018recurrent}
	McIntosh, Lane and Maheswaranathan, Niru and Sussillo, David and Shlens, Jonathon,
	Recurrent segmentation for variable computational budgets,
	Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition Workshops, {CVPR Workshop}
	(2018)
	
	\bibitem{tai2015convolutional}
	Tai, Cheng and Xiao, Tong and Zhang, Yi and Wang, Xiaogang and others,
	Convolutional neural networks with low-rank regularization,
	Proceedings of the International Conference on Learning Representations, {ICLR}
	(2016)
	
	\bibitem{li2016pruning}
	Li, Hao and Kadav, Asim and Durdanovic, Igor and Samet, Hanan and Graf, Hans Peter,
	Pruning filters for efficient convnets,
	Proceedings of the International Conference on Learning Representations, {ICLR}
	(2017)
	
	\bibitem{polino2018model}
	Polino, Antonio and Pascanu, Razvan and Alistarh, Dan,
	Model compression via distillation and quantization,
	Proceedings of the International Conference on Learning Representations, {ICLR}
	(2018)
	
	\bibitem{dong2017more}
	Dong, Xuanyi and Huang, Junshi and Yang, Yi and Yan, Shuicheng,
	More is less: A more complicated network with less inference complexity,
	Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, {CVPR}
	(2017)
	
	\bibitem{cai2018proxylessnas}
	Cai, Han and Zhu, Ligeng and Han, Song,
	Proxylessnas: Direct neural architecture search on target task and hardware,
	Proceedings of the International Conference on Learning Representations, {ICLR}
	(2019)
	
	\bibitem{tan2019mnasnet}
	Tan, Mingxing and Chen, Bo and Pang, Ruoming and Vasudevan, Vijay and Sandler, Mark and Howard, Andrew and Le, Quoc V,
	Mnasnet: Platform-aware neural architecture search for mobile,
	Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, {CVPR}
	(2019)
	
	\bibitem{netzer2011reading}
	Netzer, Yuval and Wang, Tao and Coates, Adam and Bissacco, Alessandro and Wu, Bo and Ng, Andrew Y,
	Reading digits in natural images with unsupervised feature learning,
	Proceedings of the International Conference on Neural Information Processing Systems, {NIPS}
	(2011)
	
	\bibitem{wu2016quantized}
	Wu, Jiaxiang and Leng, Cong and Wang, Yuhang and Hu, Qinghao and Cheng, Jian,
	Quantized convolutional neural networks for mobile devices,
	Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, {CVPR}
	(2016)
	
	\bibitem{han2015deep}
	Han, Song and Mao, Huizi and Dally, William J,
	Deep compression: Compressing deep neural networks with pruning, trained quantization and huffman coding,
	Proceedings of the International Conference on Learning Representations, {ICLR}
	(2016)
	
	\bibitem{Perforated}
	Michael Figurnov, Aijan Ibraimova, Dmitry Vetrov, and Pushmeet Kohli. 
	Perforated cnns: Acceleration through elimination of redundant convolutions.
	In Proceedings of the International Conference on Neural Information Processing Systems, {NIPS}
	(2016)
	
	\bibitem{luo2017thinet}
	Luo, Jian-Hao and Wu, Jianxin and Lin, Weiyao,
	Thinet: A filter level pruning method for deep neural network compression,
	Proceedings of the IEEE international conference on computer vision, {CVPR}
	(2017)
	
	\bibitem{he2017channel}
	He, Yihui and Zhang, Xiangyu and Sun, Jian,
	Channel pruning for accelerating very deep neural networks,
	Proceedings of the IEEE International Conference on Computer Vision, {ICCV}
	(2017)
	
	\bibitem{jaderberg2014speeding}
	Jaderberg, Max and Vedaldi, Andrea and Zisserman, Andrew,
	Speeding up convolutional neural networks with low rank expansions,
	British Machine Vision Conference, {BMVC}
	(2014)
	
	\bibitem{ioannou2015training}
	Ioannou, Yani and Robertson, Duncan and Shotton, Jamie and Cipolla, Roberto and Criminisi, Antonio,
	Training cnns with low-rank filters for efficient image classification,
	Proceedings of the International Conference on Learning Representations, {ICLR}
	(2016)

	\bibitem{he2016deep}
	He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian,
	Deep residual learning for image recognition,
	Proceedings of the IEEE conference on computer vision and pattern recognition, {CVPR}
	(2016)
	
	\bibitem{chen2017learning}
	Chen, Guobin and Choi, Wongun and Yu, Xiang and Han, Tony and Chandraker, Manmohan,
	Learning efficient object detection models with knowledge distillation,
	Advances in Neural Information Processing Systems, {NIPS}
	(2017)
	
	\bibitem{chen2018distilling}
	Chen, Zhenghua and Zhang, Le and Cao, Zhiguang and Guo, Jing,
	Distilling the knowledge from handcrafted features for human activity recognition,
	IEEE Transactions on Industrial Informatics
	(2018)
	
	\bibitem{hinton2015distilling}
	Hinton, Geoffrey and Vinyals, Oriol and Dean, Jeff,
	Distilling the knowledge in a neural network,
	Deep Learning and Representation Learning Workshop, {NIPS}
	(2015)
	
	\bibitem{hu2014efficient}
	Hu, Hanzhang and Grubb, Alexander and Bagnell, J Andrew and Hebert, Martial,
	Efficient feature group sequencing for anytime linear prediction,
	Proceedings of the Conference on Uncertainty in Artificial Intelligence, {UAI}
	(2014)
	
	\bibitem{krizhevsky2009learning}
	Krizhevsky, Alex and others,
	Learning multiple layers of features from tiny images,
	Citeseer,
	(2009)
	
	\bibitem{Hydranets}
	Ravi Teja Mullapudi, William R. Mark, Noam Shazeer, and Kayvon Fatahalian. 
	Hydranets: Specialized dynamic architectures for efficient inference. In The IEEE Conference on Proceedings of the Computer Vision and Pattern Recognition, {CVPR}
	(2018)
	
	\bibitem{deng2009imagenet}
	Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li,
	Imagenet: A large-scale hierarchical image database,
	Proceedings of the conference on Computer Vision and Pattern Recognition, {CVPR}
	(2009)
	
	\bibitem{gumbel1948statistical}
	Jang, Eric and Gu, Shixiang and Poole, Ben,
	Categorical reparameterization with gumbel-softmax,
	Proceedings of the International Conference on Learning Representations, {ICLR}
	(2017)
	
	\bibitem{gao2018dynamic}
	Gao, Xitong and Zhao, Yiren and Dudziak, Lukasz and Mullins, Robert and Xu, Cheng-zhong
	Dynamic channel pruning: Feature boosting and suppression,
	Proceedings of the International Conference on Learning Representations, {ICLR}
	(2018)
	
\end{thebibliography}
